The Discretely-Discontinuous Galerkin Coarse Grid for Domain Decomposition

We present an algebraic method for constructing a highly effective coarse grid correction to accelerate domain decomposition. The coarse problem is constructed from the original matrix and a small set of input vectors that span a low-degree polynomial space, but no further knowledge of meshes or continuous functionals is used. We construct a coarse basis by partitioning the problem into subdomains and using the restriction of each input vector to each subdomain as its own basis function. This basis resembles a Discontinuous Galerkin basis on subdomain-sized elements. Constructing the coarse problem by Galerkin projection, we prove a high-order convergent error bound for the coarse solutions. Used in a two-level symmetric multiplicative overlapping Schwarz preconditioner, the resulting conjugate gradient solver shows optimal scaling. Convergence requires a constant number of iterations, independent of fine problem size, on a range of scalar and vector-valued second-order and fourth-order PDEs.

==> analysis_schwarz_with_dg.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analysis of Schwarz with Coarse Grid}
\label{sec:AnalysisOfTwoLevel}




==> analysis_the_ddg_coarse_grid.tex <==
% What's my argument for why this works?
% Basically, I can show that on lowest-order regular-grid poisson,
% the DDG solve converges to a DG solve.
% For other problems, I just hope that it generalizes.
% For second order PDEs and FEM discretizations, I believe it does.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analysis of the Coarse Grid}
\label{sec:AnalysisCoarseGrid}


